NASCUP: Nucleic Acid Sequence Classification by Universal Probability

Motivated by the need for fast and accurate classification of unlabeled nucleotide sequences on a large scale, we developed NASCUP, a new classification method that captures statistical structures of nucleotide sequences by compact context-tree models and universal probability from information theory. NASCUP achieved BLAST-like classification accuracy consistently for several large-scale databases in orders-of-magnitude reduced runtime, and was applied to other bioinformatics tasks such as outlier detection and synthetic sequence generation.

==> discussion.tex <==
%!TEX root = manuscript.tex

The proposed \acl{} method performs model-based classification
using the universal probability assignment for context-tree models
from information theory. Thus, it combines the merits of existing
model-based methods and compression-based methods, which is
confirmed by its highly competitive performance in diverse datasets
in terms of time efficiency and classification accuracy.
Regardless of the number of families and the level of intra-family sequence similarity, which affected the performance of most of the alternatives, \acl~successfully maintained its accuracy, confirming its robustness
with the following advantages over the existing methods:

% To address the limitations of existing sequence classification methods,
% we propose the {nucleic acid sequence classification by universal probability} (NASCUP) method. NASCUP uses a model/feature-based approach
% with characteristics related to all three types of
% model/feature-based approaches---based on probabilistic models, $k$-mers,
% and compression---but with the following advantages over the existing methods:
% %\begin{itemize}[leftmargin=*,topsep=0em, itemsep=0em,labelsep=1em]
\begin{itemize}
	\item \textbf{Versus alignment based:} \acl~does not rely on any sequence-to-sequence comparison, and the classification time of \acl~is independent of the number of sequences per family, which enables a significant speedup. For gigabase-scale databases, such as Greengenes~\cite{desantis2006greengenes} and SILVA~\cite{quast2012silva}, many alignment-based methods would take days or even weeks for database-wide classification, whereas the time demand of \acl~is orders-of-magnitude lower.
	
	\item \textbf{Versus $k$-mer based:} NASCUP utilizes a hierarchical model called \emph{the context-tree model}, which is constructed from the ``contexts'' of training sequences using their $k$-mer information. In addition to alleviating the efficiency problem of existing $k$-mer based approaches (sparse vs.\@ dense trees) in representing the probabilistic structure of a sequence, these contexts also capture the textual information of the sequence by only keeping segments of statistical importance.
	
	\item \textbf{Versus compression based:} In deriving a good context-tree model,
NASCUP employs
the notion of minimax universal probability measure used in information theory \cite{Krichevsky--Trofimov1981, Rissanen1986, Clarke--Barron1994}.
This allows for efficient and effective modeling
and classification of multiple sequences in two stages, improving significantly upon the performance and scalability of compression
based approaches even though NASCUP shares much of their philosophical foundations.

	\item \textbf{Versus probabilistic model based:} \acl~runs faster and returns more accurate classification results than HMM-based and ICM-based alternatives. Furthermore, \acl~does not need any MSA preprocessing, which allows additional performance boosts over the HMM approaches that normally require MSA preprocessing. Compared with ICM, which also utilizes context trees, \acl~implicitly enumerates all context tree models of a given depth and traverses them so that the most probable CTM can be found (cf.~\cite{Willems--Shtarkov--Tjalkens1993, Nohre1994}).
This principled approach of tree building in NASCUP pays off with its much improved accuracy.
Even so, the running time of \acl{} typically remains lower than that of ICM.
	
\end{itemize}

As a model-based method, NASCUP can be easily adapted to test similarity between families
or a membership of a sequence or a sequence family in a group of families. We expect that
this modified version of NASCUP can be applied to problems with inherent hierarchical
structures such as taxonomy classification and phylogenetic tree construction.
A phylogenetic tree is typically constructed by measuring sequence similarities using heuristics such as progressive alignment and then by applying linkage methods to produce a dendrogram structure. In this conventional approach, results may vary (often dramatically) according to which linkage method is used.
In contrast, the modified version of \acl{} would allow direct model-to-model comparison, alleviating
the aforementioned limitations of alignment--linkage methods. Going one step further, we expect that the modified \acl{}, fully utilizing the simple Bayesian update structure of universal probability
assignments in the classification stage, will be applicable to incremental clustering, in which
an initial model is constructed from close sequences and then is incrementally augmented
by adding additional sequences.

%More technical aspects of NASCUP can be improved in the following directions,
%providing the end users with more flexibility.
%First, instead of the current classification scoring scheme of log-odds against random data,
%which is effective in many cases but cannot present an absolute criterion,
%we can adopt a more standardized scoring scheme. One such scheme can be found
%in operational taxonomic unit (OTU)~\cite{thomas2012metagenomics} binning,
%whereby a widely used threshold is 97\% similarity~\cite{stackebrandt1994taxonomic}
%at the species level.
%Second,

Instead of unidirectional contexts (that precede symbols),
we can use bidirectional contexts (that precede and succeed symbols). More generally,
the directionality of nucleotide sequences or the lack thereof can be incorporated into
modeling and classification stages. Additionally, the maximum depth of context-tree models can be
adjusted more flexibly in a data-dependent manner. A similar technique has been developed in
the context of data compression~\cite{Willems1998}, which is expected to be applicable in our
problem. The use of bidirectional contexts and adaptive maximal depths is expected to boost
accuracy further at some cost of time efficiency.

%\clearpage


==> introduction.tex <==
%!TEX root = manuscript.tex
% Intro Flow
% 시퀀스 분류는 중요한 문제다.
% 시퀀스 양은 빠르게 확대되고 있다.

% 가장 대중적인 개별적으로 시퀀스 분류하는 방법이 존재해 왔다. (BLAST and its variants)
% 그러나 이는 확장성에 한계가 있다.

% 일반적으로 한 그룹내의 시퀀스는 공통된 영역을 가지고 있다
% 따라서, 그룹내의 시퀀스는 공통된 영역의 특징으로 표현될 수 있다.
% 이렇게 모델링은 하는 방법 또한 존재해 왔다.
% 모델링 방법은 확장성은 좋지만, 좋은 모델을 만들기가 쉽지 않다.
% 
% NASCUP 접근 포인트
% (1) 확장성을 위해서: 그룹별 모델링
% (2) 기본 분류 성능을 위해서: 최적의 반복적 패턴 추출을 위한 compression 기법 도입
% 실험 결과로 제안하는 방법이 빠르고, 정확하고, 매우 확장성이 있음을 확인하였다.


\dropcap{B}iological sequence classification plays a key role
in various bioinformatics pipelines
by revealing the proximity and membership of a sequence to known sequence families~\cite{van2000virus, lu2005microrna, griffiths2005rfam, yap1993classification, tatusov2001cog}.
Expedited by new sequencing technologies, the amount of biological information is growing rapidly, making the need for having an effective classification method more important than ever.
Existing methods, however, often suffer from common limitations in time and space efficiency
of training and testing, classification accuracy, or scalability.


Common approaches for sequence classification can be
broadly grouped into two categories---alignment-based and model/feature-based ones.
In alignment-based approaches the similarity between a query sequence and the sequences in a database is measured by sequence-to-sequence alignment,
which can be then used to determine the class of the query sequence.
Widely used alignment tools include BLAST~\cite{blast}, FASTA~\cite{pearson19905}, BLAT~\cite{kent2002blat}, SOAP~\cite{li2008soap}, USEARCH~\cite{edgar2010search}, UBLAST~\cite{edgar2010search}, and caBLAST~\cite{loh2012compressive}. As the size of the database grows, the time demand for databasewide classification often becomes prohibitively costly. To address this challenge, various speedup techniques have been proposed (\eg, seed-and-extend~\cite{blast, pearson19905}, in-memory processing~\cite{kent2002blat, li2008soap}, word-counting based prioritizing~\cite{edgar2010search}, and database compression~\cite{loh2012compressive}), which, however,  typically sacrifice accuracy for efficiency.

In general, sequences within a family share highly conserved regions that have been maintained relatively unchanged by natural selection. 
Thus, a sequence family can be represented with the repetitive sequence patterns or distributions that can be distinguished from other families.
In model/feature-based approaches, a model is derived from the sequences in a family and perform sequence-to-model comparison in order to classify query sequences. 
Several types of model/feature-based methods exist. 
Probabilistic model based hidden Markov models (\eg, HMMER~\cite{nhmmer, eddy2011accelerated, eddy1998profile} and interpolated context model (ICM)~\cite{icm}
(\eg, GLIMMER~\cite{glimmer} and Phymm~\cite{phymm}), $k$-mer based approaches, such as RDP~\cite{methodRDP}, and Compression-based approaches~\cite{kocsor2006application, loewenstern1995dna} have been used.
In the aspect of classification stage, sequence-to-model comparison is much more scalable than sequence-to-sequence comparison. However, modeling to represent the characteristics of sequences is not easy and sometimes takes an excessive amount of running time.

For scalability and classification performance, we tried to build a model-based methods by using the good proxy, universal probability.
% To exploit the repetitive patterns or their distribution, we tried to use compression technique.
% Compression has traditionally been used to represent the original data in fewer bits and, in the procedure, the most compressive repeated patterns are replaced with shortest bits.



% Several types of model/feature-based methods exist. First, probabilistic model-based approaches derive a model from the sequences in a family and perform sequence-to-model comparison in order to classify query sequences.
% Classification techniques based on hidden Markov models (\eg, HMMER~\cite{nhmmer, eddy2011accelerated, eddy1998profile} and SAM-T97~\cite{karplus1998hidden}),
% despite their popularity, often suffer from excessive running time caused by iterative training of the model and preprocessing by multiple sequence alignment (MSA).
% Techniques based on the interpolated context model (ICM)~\cite{icm}
%  (\eg, GLIMMER~\cite{glimmer} and Phymm~\cite{phymm}) show improved time efficiency but often fail to achieve the desired accuracy
%  due to the greedy nature in their search strategy.

% Second, $k$-mer based approaches, such as RDP~\cite{methodRDP}, NBC~\cite{NBC}, Kraken~\cite{wood2014kraken}, and CLARK~\cite{ounit2015clark},
% extract $k$-mer counts from the data and then perform classification using the acquired $k$-mer spectra.
% On the theoretical side, these methods involve somewhat arbitrary metrics for comparison of $k$-mer spectra, such as the Euclidean distance.
% On the practical side, the need for storing and processing $k$-mer data often limits the scalability and efficiency of many $k$-mer based methods.

% Compression-based approaches~\cite{kocsor2006application, loewenstern1995dna} constitute the third, and the least popular, type of model/ feature-based methods.
% Roughly speaking, these approaches utilize the marginal description complexity of a query sequence when it is compressed as a sequel to database sequences;
% if the query sequence belongs to the family, then it would be compressed efficiently. The lack of a separate modeling process and the difficulty of compressing all sequences in a family limit the wide adoption of these techniques,
% not to mention their relatively poor accuracy.



% To address the limitations of existing sequence classification methods,
% we propose the {nucleic acid sequence classification by universal probability} (NASCUP) method. NASCUP uses a model/feature-based approach
% with characteristics related to all three types of
% model/feature-based approaches---based on probabilistic models, $k$-mers,
% and compression---but with the following advantages over the existing methods:
% %\begin{itemize}[leftmargin=*,topsep=0em, itemsep=0em,labelsep=1em]
% \begin{itemize}
% 	\item \textbf{Versus alignment based:} \acl~does not rely on any sequence-to-sequence comparison, and the classification time of \acl~is independent of the number of sequences per family, which enables a significant speedup. For gigabase-scale databases, such as Greengenes~\cite{desantis2006greengenes} and SILVA~\cite{quast2012silva}, many alignment-based methods would take days or even weeks for database-wide classification, whereas the time demand of \acl~is orders-of-magnitude lower.
	
% 	\item \textbf{Versus $k$-mer based:} NASCUP utilizes a hierarchical model called \emph{the context-tree model}, which is constructed from the ``contexts'' of training sequences using their $k$-mer information. In addition to alleviating the efficiency problem of existing $k$-mer based approaches (sparse vs.\@ dense trees) in representing the probabilistic structure of a sequence, these contexts also capture the textual information of the sequence by only keeping segments of statistical importance.
	
% 	\item \textbf{Versus compression based:} In deriving a good context-tree model,
% NASCUP employs
% the notion of minimax universal probability measure used in information theory \cite{Krichevsky--Trofimov1981, Rissanen1986, Clarke--Barron1994}.
% This allows for efficient and effective modeling
% and classification of multiple sequences in two stages, improving significantly upon the performance and scalability of compression
% based approaches even though NASCUP shares much of their philosophical foundations.

% 	\item \textbf{Versus probabilistic model based:} \acl~runs faster and returns more accurate classification results than HMM-based and ICM-based alternatives. Furthermore, \acl~does not need any MSA preprocessing, which allows additional performance boosts over the HMM approaches that normally require MSA preprocessing. Compared with ICM, which also utilizes context trees, \acl~implicitly enumerates all context tree models of a given depth and traverses them so that the most probable CTM can be found (cf.~\cite{Willems--Shtarkov--Tjalkens1993, Nohre1994}).
% This principled approach of tree building in NASCUP pays off with its much improved accuracy.
% Even so, the running time of \acl{} typically remains lower than that of ICM.
	
% \end{itemize}

We have performed a set of comprehensive experiments that test \acl~with alignment-based methods (BLAST and its variants) and model-based methods (HMMER, RDP, ICM, and gzip) on a variety of real sequence datasets for functional non-coding RNA classification, microbial taxonomy classification, 
and binary coding/non-coding RNA classification.
Our experimental results confirm the effectiveness of \acl~and its advantages over existing state-of-the-art in terms of time, accuracy, and scalability.




==> methods.tex <==
%!TEX root = manuscript.tex



\newcommand{\ttA}{\texttt{A}}
\newcommand{\ttC}{\texttt{C}}
\newcommand{\ttG}{\texttt{G}}
\newcommand{\ttT}{\texttt{T}}
\newcommand{\ttS}{\texttt{*}}
\newcommand{\bn}{\mathbf{n}}
\newcommand{\bm}{\mathbf{m}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\nts}{\texttt{A},\texttt{C},\texttt{G},\texttt{T}}
\newcommand{\btheta}{\boldsymbol{\theta}}
\newcommand{\balpha}{\boldsymbol{\alpha}}
\newcommand{\argmax}{\operatornamewithlimits{argmax}}
\definecolor {shade}{rgb}{0.9,0.9,0.9}


NASCUP aims to extract the structure of each nucleotide sequence family
by relative frequencies of the symbols \nts (\texttt{U}) in the
constituent sequences (model building) and utilize this structural information to
assign the query sequence to the best fit family (classification).
Unlike the simplistic $k$-mer approach, however, NASCUP leverages the notion of
\emph{universal probability} in both variable-order Markov model building and classification pipelines.



\subsection*{Universal Probability}

% \begin{figure*}[t!]
% \vspace{-0.75em}
%   \centering
%   \includegraphics[width=\textwidth]{overview}
% %  \caption{Context graph with depth 2 and the model-building process for a single database sequence X=\texttt{CGCACTCCGTCG}.}
%   \caption{Context graph with depth 2 and the context-tree model for sequence X=\texttt{CGCACTCCGTCG} [solid and dotted lines: selected and pruned contexts, respectively; the set of \colorbox{shade}{shaded regions}: the optimal CTM found]. }  \label{fig:model_building}
% \end{figure*}

\begin{figure}[t!]
\vspace{-0.75em}
  \centering
  \includegraphics[width=0.45\textwidth]{ctm_small}
%  \caption{Context graph with depth 2 and the model-building process for a single database sequence X=\texttt{CGCACTCCGTCG}.}
  \caption{Context graph with depth 2 and the context-tree model for sequence X=\texttt{CGCACTCCGTCG} [solid and dotted lines: selected and pruned contexts, respectively; the set of \colorbox{shade}{shaded regions}: the optimal CTM found]. }  \label{fig:model_building}
\end{figure}

The theory of universal probability has been developed
in ergodic theory, information theory, and online learning.
Roughly speaking, a universal probability distribution $Q$ approximates
all distributions $P$ in a given class of distributions uniformly well
and thus serves as a simultaneously good proxy.
The existence and construction of such universal probability distributions
are well-known for bounded parametric families \cite{Rissanen1986, Clarke--Barron1994}.
In particular,
the conditional Krichevsky--Trofimov probability $Q$ (details discussed shortly
in Section 2.3)
can approximate any $L$-state quaternary stationary Markov process $P$ with
\[
\frac{1}{n} \log \frac{P(x^n)}{Q(x^n)} \sim \frac{3L}{2} \frac{\log n}{n} \to 0 \quad\text{as } n \to \infty
\]
uniformly in $x^n$ with very reasonable lower-order terms.
The famous Lempel--Ziv incremental parsing algorithm \cite{Ziv--Lempel1978}
used in data compression can be recast as an assignment of probability
that is universal with respect to the class of all finite-alphabet stationary ergodic processes
with less sharp convergence properties.

\subsection*{Variable-order Markov (VOM) Models}

The simplest class of probability models
considered in bioinformatics and other scientific disciplines
is the class of $k$-mer models
(see, for example,~\cite{methodRDP, NBC, wood2014kraken, ounit2015clark})
or equivalently the class of Markov models of depth $d = k-1$. Albeit straightforward to theorize and efficient to implement,
the generic class of $d$-th order Markov processes suffers from the large number of states (also called \emph{contexts})---4096 contexts at depth 6---most of which do not appear in a sequence,
and the small number of occurrences of each context, which may
not contribute to any statistically meaningful structure and instead cause unnecessary overfitting. 

NASCUP thus considers the class of \emph{context-tree models} (CTMs), which
% is used widely in ICM~\cite{icm} and its variations~\cite{glimmer,phymm}.
is used in ICM~\cite{icm}.
We start with a context graph
(as shown in Fig.~\ref{fig:model_building} for $d = 2$) that consists of nodes representing
all potential contexts $\{\nts, \ttS\}^d$, where $\ttS$ denotes ``don't care.''
Any subtree of this context graph is called a context-tree model, whose contexts (leaf nodes) represent
the reduced set of Markov states (clumped together from all possible $4^d$ states).
When a given context-tree model only has contexts of the form $\{\ttS\}^j \times \{\nts\}^{d-j}$ for some $j$, it is referred to as a variable-order Markov (VOM) model.  




% \begin{figure*}[t!]
% \vspace{-0.75em}
%   \centering
%   \includegraphics[width=\textwidth]{overall_flow}
% %  \caption{Context graph with depth 2 and the model-building process for a single database sequence X=\texttt{CGCACTCCGTCG}.}
%   \caption{Overall flow of ~\acl. The proposed \acl~methodology consists of two main steps: (1) Model-building, (2) Classification.}  \label{fig:overall_flow}
% \end{figure*}

\begin{figure}[t!]
\vspace{-0.75em}
  \centering
  \includegraphics[width=0.45\textwidth]{flow2}
%  \caption{Context graph with depth 2 and the model-building process for a single database sequence X=\texttt{CGCACTCCGTCG}.}
  \caption{Overall flow of ~\acl. The proposed \acl~methodology consists of two main steps: (1) Model-building, (2) Classification.}  \label{fig:overall_flow}
\end{figure}

%In the following, we provide the details on how NASCUP works.

\subsection*{Model Building}

% NASCUP builds a context-tree model (CTM) for each sequence family in the given dataset.
In the model building stage, NASCUP finds the best CTM for each family of sequences by
finding the CTM that maximizes the
\emph{universal probability} with respect to
all distributions under the CTM. This maximum likelihood model selection
approach is well justified by statistics and information theory,
with our variation being the use of the universal probability
as a minimax optimal representative for a class of potential distributions.
In case the class of candidate CTMs is limited
to VOM models, the universal probability maximization can be performed recursively,
as demonstrated earlier by~\cite{Willems--Shtarkov--Tjalkens1993, Nohre1994} for data compression applications.


{\bf Step 1: Symbol counting for each context}.
NASCUP initially counts the nucleotide symbols \nts{}
that follow each of length-$d$ contexts in $\{\nts\}^d$ by
enumerating all $k$-mers ($k = d+1$) from all sequences in the family.
These counts are then merged bottom--up along the context graph of depth $d$.
% as shown in Figure~\ref{fig:model_building}.
% above removed...
The context graph has as its nodes $5^d$ contexts
that include the ``don't care'' ($\ttS$) symbol in addition to $\nts$,
with $\ttS\ttS\cdots\ttS$ being the root (depth $0$) and physical contexts from $\{\nts\}^d$ being $4^d$ leaves
at the bottom (depth $d$). Each context from depth $0$ to $d-1$ is branched into one or more sets of children
in the next depth by replacing each $\ttS$ symbol with a set of $\nts$.
%The root has $d$ sets of children.
%% one of
%More generally, a context with $j$ $\ttS$ symbols has $j$ sets of children.
%For example, context $*\texttt{A}$ at depth $1$ is branched into one children set $\texttt{AA}, \texttt{CA}, \texttt{GA}, \texttt{TA}$ at depth 2, and $\texttt{AA}$ at depth 2 is, in turn, connected to two parents
%$\ttS\ttA$ and $\ttA\ttS$.
The counts of the symbols at each context $s \in \{\nts,*\}^d$ is denoted as $n_i(s)$, $i \in \{\nts\}$,
which are collectively written as a 4-dimensional count vector $\bn(s)$, \eg,
%For example,
\[
\begin{aligned}
\bn(\ttS\ttS) &= \bn(\ttS\ttA) + \bn(\ttS\ttC) + \bn(\ttS\ttG) + \bn(\ttS\ttT). %\\
 %       &= \bn(\ttA\ttS) + \bn(\ttC\ttS) + \bn(\ttG\ttS) + \bn(\ttT\ttS).
\end{aligned}
\]


{\bf Step 2: Universal probability assignment to each context.}
It is well known that the Krichevsky--Trofimov (KT)~\cite{Krichevsky--Trofimov1981} probability
distribution is asymptotically minimax universal with respect to i.i.d.\@ processes
with unknown parameters~\cite{Rissanen1986, Clarke--Barron1994}
and is used widely in universal data compression~\cite{Cover--Thomas2006}.
Hence, given $\bn = \bn(s)$ for each context $s$, NASCUP computes
the Krichevski--Trofimov (KT)~\cite{Krichevsky--Trofimov1981}
probability
\begin{equation}
\begin{aligned}
Q^{\textrm{KT}}(s)
&= Q^{\textrm{KT}}(n_\texttt{A},n_\texttt{C},n_\texttt{G},n_\texttt{T})\\
&= \frac{ \prod_{i\in \{\texttt{A},\texttt{C},\texttt{G},\texttt{T}\}} \prod_{j_i=1}^{n_i} (j_i - 1/2) }
{ \prod_{j=1}^{n_\ttA + n_\ttC + n_\ttG + n_\ttT} (j + 1)},
\label{eq:kt}			
\end{aligned}
\end{equation}
which can be viewed as a Dirichlet mixture of
independent and identically distributed (i.i.d.) random processes over the quaternary alphabet. 

%where an empty product is set to 1 by convention.

{\bf Step 3: Recursive context tree maximization.}
For a context tree model with a set $S$ of contexts, \eqref{eq:kt} results in the probability
of the entire sequence (or sequence family) given by
\begin{equation} \label{eq:kt-sequence}
\prod_{s \in S} Q^\textrm{KT}(s).
\end{equation}
This \emph{conditional} KT probability distribution continues to be minimax universal (see, for example,~\cite{Rissanen1986, Willems--Shtarkov--Tjalkens1993}), if computed with the correct context tree model. NASCUP finds the best context tree model, or equivalently, $S$ that maximizes~\eqref{eq:kt-sequence} recursively by
starting with the root node in the context graph in a depth-first manner
and computing for each context $s$
\begin{equation}
Q(s) = \max \bigl\{ Q^\textrm{KT}(s),\,
\max_{\textrm{children sets of $s$}} {\textstyle\prod\limits_{\textrm{child $s'$ in each set}}}
Q(s') \bigr\},
\label{eq:maximizing}
\end{equation}
where the inner maximum is over different children sets of $s$.
If $s$ is a leaf (at depth $d$), then $Q(s) = Q^\textrm{KT}(s)$. As an example,
for $d = 2$,
\begin{align*}
Q(\ttS\ttS)
&= \max\{ Q^\textrm{KT}(\ttS\ttS),\,
Q(\ttS\ttA)Q(\ttS\ttC)Q(\ttS\ttG)Q(\ttS\ttT)\}, \\ %,\, \\
%& \phantom{blankblankblackbl{ }} Q(\ttA\ttS)Q(\ttC\ttS)Q(\ttG\ttS)Q(\ttT\ttS) \}, \\
Q(\ttS\ttA) &= \max\{ Q^\textrm{KT}(\ttS\ttA), \,
Q^\textrm{KT}(\ttA\ttA)Q^\textrm{KT}(\ttC\ttA)Q^\textrm{KT}(\ttG\ttA)Q^\textrm{KT}(\ttT\ttA) \}.
\end{align*}%
Each children set that does not attain the maximum is pruned.
In case of a tie between a parent context and its children set,
we choose the parent for the sparsity of the resulting model.
Upon completion of this maximizing and pruning step,
the remaining nodes of the graph is either a leaf or a non-leaf with
a single non-overlapping set of four children.
This tree and the count vectors of its nodes (contexts) form the
context-tree model (CTM) for the given sequence family.

\subsection*{Classification}
The notion of universal probability is utilized in the classification stage as well.
For simplicity, consider two families of sequences with true distributions $P_1$
and $P_2$, and two universal probability distributions $Q_1$ and $Q_2$, each corresponding to
the best CTM for a given family selected in the model building stage.
Let $\by_1$ and $\by_2$ be the sequences (collectively) in each family and $\bx$
be the query sequence we wish to classify. Were $P_1$ and $P_2$ known, then
the optimal Bayes classifier would compare
\[
\log P_j(\bx), \quad j = 1,2,
\]
and choose the one with the maximum likelihood---or compute their ratio (log-likelihood ratio)
and classify according to some threshold.
If we assume that the correct CTMs were found, then
\begin{equation} \label{eq:univ-classification}
\log Q(\bx|\by_j) \approx \log P_j(\bx|\by_j) \approx \log P_j(\bx), \quad j = 1,2,
\end{equation}
where the conditional probabilities denote those
of the concatenated sequence, say, $Q(\by_j, \bx)$,
divided by the probability of the sequence, say, $Q(\by_j)$.
Here the first approximation is justified by the universality of $Q$ and
the second approximation is justified by the Markovity of $P_j$.
Hence, approximately we can perform Bayes classification or any log-likelihood ratio test
even without knowing the true probability distributions!
The idea of using universal probability in classification
traces back to~\cite{Ziv1988, Gutman1989} and NASCUP extends it to
CTMs and associated minimax universal probability distributions.

Note that the measure, $-\log Q(\bx|\by_j)$, can be interpreted as
the length of the optimal source code for the distribution $Q$ \cite{Cover--Thomas2006}.
In this sense, NASCUP can be viewed as a refinement of compression-based
classification methods~\cite{kocsor2006application, loewenstern1995dna}
that uses the optimal source code using universal probability.

Assume that there are $K$ known families of sequences in the database
and that NASCUP has already constructed context-tree models for them.
Given an unlabeled input sequence $\bx$, NASCUP computes the membership scores
of the sequence for the $K$ context-tree models in three steps.

{\bf Step 1. Symbol counting for each context.}
As in the modeling stage, NASCUP performs $(d+1)$-mer enumeration on $\bx$
to generate count vectors $\bm(s) = (m_\texttt{A}(s),m_\texttt{C}(s),m_\texttt{G}(s),m_\texttt{T}(s))$.
%for each possible context $s$ of length $d$.

{\bf Step 2. Universal probability computation for each family.}
Fix a context-tree model $M$
characterized by a context tree (a set $S$ of contexts) and
the count vectors $\bn(s)$ for $s \in S$.
Following~\eqref{eq:univ-classification},
NASCUP computes the conditional probability of $\bx$ given $M$ as
\begin{equation}
Q(\bx|M) = \prod_{s \in S} Q(\bm(s) | \bn(s)),
\end{equation}
which is computed
again according to the KT probability assignment in~\eqref{eq:kt},
which has a simple Bayesian update for
the conditional probability computation:
\begin{equation}
Q(\bm|\bn) = \frac{Q^\textrm{KT}(\bm + \bn)}{Q^\textrm{KT}(\bn)}.
\label{eq:conditional_kt}
\end{equation}

{\bf Step 3. Finding the best model.} NASCUP compares the conditional probabilities in~\eqref{eq:conditional_kt} over all $K$ families
and selects the family with the largest probability.


% Fig.~\ref{A-fig:frog} temp supporting information testing



==> results.tex <==
%!TEX root = manuscript.tex

% \subsection*{Setup and Datasets}
% \input{tab-data}

% \def\CC{{C\nolinebreak[4]\hspace{-.01em}\raisebox{.35ex}{\tiny\bf ++}}}

% We implemented \acl~in \CC{}
% and measured its performance in terms of runtime (\ie, modeling time plus classification time),
% and classification accuracy with 10-fold cross validation, using a linux machine (Ubuntu 12.04, 2.2 GHz Intel Xeon E5-4620, and 512 GB memory) without any parallelization.
% For comparison, we also prepared the implementations of nine alternatives: BLAST, HMMER, ICM, gzip, RDP, USEARCH, UBLAST, caBLAST, and BLAT.

% For BLAST and its variants (USEARCH, UBLAST, caBLAST, and BLAT), nearest-neightbor classification was carried out. For gzip, the class of a query sequence was determined as the family whose compressed representation showed the smallest difference with and without the query.

% We used nine datasets of three types: functional non-coding RNAs, microbial taxonomy, and coding/non-coding RNAs (\tablename~\ref{tab:data}).

% For the first type, we used Rfam~\cite{rfam}, a database of functional RNA families of rRNAs, tRNAs, miRNAs, siRNAs, and cis-regulatory elements. For the second type, we used databases of rRNA sequences (RDP~\cite{methodRDP}, Greengenes~\cite{desantis2006greengenes}, and SILVA~\cite{quast2012silva}) and pyrosequencing datasets (Artificial~\cite{quince} and Divergent~\cite{quince}). SILVA consisted of two subsets, one from large subunit (LSU) 23S and 28S rRNA sequences and the other from small subunit (SSU) 16S and 18S sequences. The two pyrosequencing datasets contained mixtures of microbial 16S rRNA sequenced with the 454 technology. %As ground truth, \textcolor{black}{We grouped the taxonomy of the rRNA sequences at the genus level.} The ground truth for the pyrosequencing datasets was calculated using the Smith-Waterman algorithm~\cite{smith1981identification} to reference sequences.
% For the third type, we used (non)coding RNA sequences from RefSeq~\cite{ncbi}, Rfam~\cite{rfam}, and Ensembl~\cite{flicek2013ensembl}.

% As preprocessing, we ignored the sequences containing symbols other than \texttt{ACGT(U)} and, for 10-fold cross validation, excluded the sequence families with less than ten sequences for all datasets.
% Since some methods compared could not handle large data in reasonable time, we reduced the data as follows: First, for Rfam and rRNA databases, we limited the maximum number of sequences in each family to 2,000 by random sampling. For Greengenes and SILVA, we further modified the samples by cd-hit-est~\cite{li2006cd} using the 97\% similarity threshold~\cite{stackebrandt1994taxonomic}.
% For RDP and CN, we downloaded the public datasets used by mothur~\cite{schloss2009introducing} and RNAcon~\cite{panwar2014prediction}, respectively, and preprocessed them as above.
% %For HS, we limited the sequence length from 20 to 16,000.

% The source code and test data are available at http://data.snu.ac.kr/nascup.


% \subsection*{\acl~Performance Evaluation }

% \begin{figure*}[t!]
% \centering
% \includegraphics[width=0.98\textwidth]{res_depth}
% \caption{Performance evaluation of \acl: (A) Classification accuracy. (B) The number of contexts in the model. Each point in a plot represents the average of 10-fold cross validation results. The datasets in the $x$-axes for (A) and (B) were listed in the order of the average pairwise distance between sequences within a family} 
% \label{fig:r_depth}
% \end{figure*}


% We evaluated the performance of NASCUP on the nine datasets in Table~\ref{tab:data} in terms of accuracy (the ratio of the numbers of correct classifications and total queries), memory usage, and running time, as shown in Fig.~\ref{fig:r_depth}. As the depth parameter $d$
% directly affects the performance of NASCUP as the basic unit of context counting and tree building, we measured the performance as varying $d$ from 3 to 8.

% Fig.~\ref{fig:r_depth}(a) shows the accuracy of NASCUP for each dataset for different values of $d$. Note that the datasets labeled in the $x$ axis of the plot are arranged in the decreasing order of the average intra-family distance (AIFD, the normalized pairwise distance between the sequences within a family). We can observe two patterns in this plot. First, the accuracy improved by increasing $d$ to some extent but eventually became saturated (in this experiment, there were negligible improvements by using $d \ge 6$). Using an unnecessarily large value of $d$ would thus incur time and space inefficiency and overfitting with no performance gain. Second, the accuracy of NASCUP depended on AIFD, giving higher accuracy for datasets with lower AIFD, as expected from the fact that a family consists of more diverse sequences (higher AIFD) would typically make family classification more challenging.

% Fig.~\ref{fig:r_depth}(b) presents the number of contexts (\ie, leaf nodes) in the model for each dataset. Having fewer contexts will be helpful in reducing the memory usage and for expediting classification. The conventional $k$-mer counting would give a CTM with $4^d$ contexts, which may be prohibitively large for large $d$. For NASCUP, the number of contexts also grew for increasing $d$, as shown in the plot. However, as we increased $d$, NASCUP produced substantially fewer contexts than the conventional $k$-mer counting. For instance, for $d=8$, there was 95\% reduction in the leaf count by using NASCUP (see the dotted line representing the number of contexts for vanilla $k$-mer counting with $d=8$). The dependency of the context counts on data was as strong as that on $d$, but NASCUP tended to produce more contexts for HS and CN (the two with high AIFD), especially for larger $d$ values.

% Figs.~\ref{fig:r_depth}(c) and~\ref{fig:r_depth}(d) show the running time of NASCUP for modeling and classification, respectively. Note that these plots use a different ordering for the dataset labels in the $x$-axes; the labels are now sorted in the ascending order of the number of sequences in a dataset. Using higher $d$ resulted in higher modeling and classification time. Recall that the model size will grow exponentially in $d$, directly affecting the time demand for $k$-mer counting and computation of $Q^\text{KT}$ and $Q$. The running time also grew as we used datasets with more sequences and sequence families.

% These results suggest that using $d=6$ would best balance accuracy and running time,
% which will be used in the following experiments.


% \subsection*{Performance Comparison with Other Classification Methods}
% \subsection*{Performance Comparison on Dataset Diversity}


% \input{tab-result}

% \input{tab-time}

% \begin{figure*}
% \centering
% \includegraphics[width=1\textwidth]{res_top}
% \caption{Performance comparison between \acl~and the four main alternatives [Each result represented in the order of \acl, BLAST, USEARCH, HMMER and RDP.
% BLAST and HMMER are the most commonly used methods in each field. USEARCH showed the second best accuracy within alignment-based methods and RDP showed the best performance within the model/feature-based methods.] (a) Classification accuracy. (b) Classification time.}
% \label{fig:res_compare_with_others}
% \bigskip
% \end{figure*}

Datasets used in our experiments came from a variety of sources, and their families are organized on a functional or taxonomic basis with varying similarity degrees. 
Even with these diversity, \acl~and BLAST showed robust performance over all datasets, maintaining mean accuracy over 0.95, unlike the other methods whose performance varied often significantly over data as detailed in \tablename~\ref{tab:result}. HMMER showed good performance on RF but not in microbial datasets, and RDP worked well on microbial datasets but it showed unsatisfactory results on functional RNAs. 

% Figs.~\ref{fig:res_compare_with_others}(a) and~\ref{fig:res_compare_with_others}(b) respectively show the total runtime (\ie, modeling plus classification) and the classification time of \acl~and the other methods. Since modeling occurs once but classification runs multiple times, we plotted the classification time separately.

\acl, RDP, and USEARCH ran significantly (often by orders of magnitude) faster for most of the data, as detailed in \tablename~\ref{tab:result}. The overall performance of RDP and USEARCH, however, did not match that of \acl~in terms of (both arithmetic and geometric). 


% The accuracy of RDP, ICM, gzip, and HMMER was lower than 80\% for three or more datasets. For RF (which has more than 1,000 families), the accuracy of RDP and caBLAST was only about 50\% and 40\%, respectively. USEARCH, UBLAST, caBLAST, and BLAT showed unsatisfactory results for CN, giving the accuracy of under 30\%.

%\clearpage

\subsection*{Scalability}
%Fig.~\ref{fig:res_time}
With the development of sequencing and bioinformatic analysis technology, the number of biological sequences is growing rapidly, and new families are discovered and created. 
As the demand for scalability, we conducted two types of scalability test; one for expanding the number of DB sequences and the other for expanding the number of newly discovered families.

%Given that \acl, BLAST, and USEARCH were the three most accurate methods,
%we further compared them in terms of scalability. 
Before comparing NASCUP with the other methods, we first tested how the modeling and classification times of \acl~were affected as the database size grew. To this end, we gradually increased the number of sequences sampled from the full GG data (from 60,717 to 560,969 sequences) and fixed the numbers of query sequences and families to 5,000 and 1,040, respectively. \figurename~\ref{fig:res_time}(a) shows the measured modeling time and classification time. As expected, the modeling time grew as the size of dataset increases. On the other hand, the classification time grew only marginally since it is almost independent of the number of sequences in a family, once the modeling has been completed. This feature makes \acl~scalable to large data, as is shown in \figurename~\ref{fig:res_time}(b) that the total runtime of \acl~is orders of magnitude lower than that of BLAST regardless of the data size. For the smallest data, USEARCH was faster than \acl, but as the dataset size grew, \acl~consistently outperformed USEARCH in running time, and the performance gap between the two became wider.

To see the scalability in families, we increased every 100 new families to existing families and fixed the number of query sequences to 5,000. As represented in \figurename~\ref{fig:res_time}(c), the modeling time did not increased because \acl~ only run the modeling procedure for newly added families and the classification time grew as the total number of families increases. Likewise in \acl~, HMMER, family unit modeling methods, showed similar runtime pattern represented in \figurename~\ref{fig:res_time}(d). 
The sequence-to-sequence comparison classifiers were only affected by the total number of sequences, since there is no modeling process. 
The discriminative learning based methods, such as SVM, random forest, require full training even though only one new family is discovered; continual learning concept is hard to applied.


\begin{figure*}[t!]
\centering
\includegraphics[width=1\textwidth]{res_bgg4}
\caption{Scalability tests using the Greengenes~\cite{desantis2006greengenes} database and its subsets: (a) Modeling throughput vs classification throughput of \acl. (b) Variation of total throughput of \acl, BLAST and HMMER over the data size. (throughput: the number of processed sequences per second of time)
}
\label{fig:res_time}
\end{figure*}

\subsection*{Robustness in noise database}

Sequence label is assigned by domain experts or certain programs without knowing the real ground truth.
% , so it is hard to say that every sequences is correctly specified.
Therefore, we assumed that there are mislabeled sequences in the existing database, and tested the classification by increasing the mis-labeling ratio from 1\% to 20\%, represented in \figurename~\ref{fig:noise}.
\acl~showed strong robustness with little performance degradation even in 20\% of noise database, unlike other methods whose performance degraded as the noise ratio increases.


\begin{figure*}[t!]
\centering
\includegraphics[width=1\textwidth]{res_noise}
\caption{Robustness in noise database between \acl, BLAST and HMMER: (a) Variation of accuracy in noised RF, (b) Variation of accuracy in noised GG. (HMMER had a model-building error between noise ratio 10\% and 20\% due to no consensus columns)}
\label{fig:noise}
\bigskip
\end{figure*}


\subsection*{One-Class Classification}

\begin{figure}[t!]
\centering
\includegraphics[width=0.45\textwidth]{res_outlier}
\caption{Outliers detection in staphylococcus [The number of sequences in the staphylococcus and others is 10,390 and 1,039 respectively. The outliers were from each of the 1,039 other genus-level families except staphylococcus.]: (a) Distribution of staphylococcus and others on cross-entropy in \acl, (b) PR curves and AUC values in \acl~and HMMER.}
\label{fig:outlier}
\bigskip
\end{figure}

For discriminative classification approaches, one-class classification is a very challenging problem because it should identify whether a sequence belongs to the target class, with only the target class data given.
\acl~builds a generative model for each family independently; it does not need any adversarial discriminative data. 
we tried one-class classification for outlier detection in staphylococcus and compared its performance with HMMER. \figurename~\ref{fig:outlier}a shows the distribution of cross-entropy values in staphylococcus and outliers, and \figurename~\ref{fig:outlier}b shows PR curves and AUC. The number of false predictions (others considered staphylococcus) in \acl~and HMMER is 6 and 768 respectively, based on TRP 100\%.

\subsection*{Possibility as Preprocessor for Hybrid Methods }
Due to the rapidly growing databases, the sequence-to-sequence approaches may require a model-based classifier as a preprocessor to ensure scalability. 
To see the possibility as a preprocessor, we checked the accuracy of \acl~as extending the TOP rank besides the TOP 1. 
Extending the TOP rank to TOP 10, \acl~could acquire over 99\% accuracy in all datasets used. 
enormously reduce the search space.
if we use top 10 families as candidate we could reduce the search space enormously.


% \begin{figure*}[t!]
% \centering
% \includegraphics[width=1\textwidth]{res_outlier_dist2}
% \caption{Distribution of staphylococcus with outliers: (a) Distribution in HMMER on cross-entropy, (b) Distribution in GMM on minus log-probability, (c) Distribution in OneClassSVM on minus distance, (d) Distribution in \acl~on cross-entropy.}
% \label{fig:outlier_dist}
% \bigskip
% \end{figure*}


% The bottom line from our experiments can be summarized as follows: \acl~and BLAST were the two \emph{universal} tools that showed satisfactory performance on all the datasets. However, \acl~was the only \emph{scalable} tool that could process large-scale data efficiently and accurately.




==> tab-methods.tex <==

\begin{spacing}{1.1}
\setlength{\tabcolsep}{16pt}

\ctable[
    caption = {  },
    label = tab:method,
    pos=htbp,
    star,
    doinside = \footnotesize
]{rcccc}{
%\tnote[$\ast$] {\acl-7 means depth of 7 which is comparable to $8$-mer.\\\acl-6 means depth of 6 which is comparable to $7$-mer.}
}{
    \toprule
          & purpose & algorithm & comparison type & score \\
    \midrule
    \multirow{3}[3]{*}{NASCUP} & \multirow{3}[3]{*}{general} & probabilistic
& \multirow{3}[3]{*}{sequence-to-model} & O \\
 & & k-mer & & \\
 & & compression & & \\
 \midrule
    BLAST & \multirow{5}[5]{*}{general} & \multirow{4}[5]{*}{alignment} & \multirow{4}[8]{*}{sequence-to-sequence} & O \\
    USEARCH &       &       &       & O \\
    UBLAST &       &       &       & O \\
    BLAT  &       &       &       & O \\
    caBLAST &       & compression
& sequence-to-model  & O \\
          &  & alignment & sequence-to-sequence & \\
 \midrule
    HMMER & functional DB
 & probalistic & sequence-to-model & O \\
 & remote homologs & & & \\
 \midrule
    RDP   & \multirow{5}[5]{*}{metagenome} & k-mer & \multirow{3}[3]{*}{sequence-to-model} & O \\
    Phymm &       & probabilistic &       & O \\
    QIIME2 &       & k-mer &       & O \\
    \cmidrule{3-5}
    UCLUST &       & clustering & \multirow{2}[2]{*}{sequence-to-sequence} & O \\
    Mothur &       & clustering &       & O \\
    \midrule
    gzip  & general & compression & sequence-to-model & compressed size \\
    \bottomrule
}
\end{spacing}


